Constraining the Coronal Heights and Readjustment Velocities Based on the Detection of a Few Hundred Seconds Delays in the Z Source GX 17+2

Neutron star Z type sources provide a unique platform in order to understand the structure of accretion disk-corona geometry emitting close to the Eddington luminosity. Using RXTE and NuSTAR satellite data, we performed cross correlation function (CCF) studies in GX 17+2 in order to constrain the size of corona responsible for hard X-rays. From the RXTE data, we found that during horizontal and normal branches, the CCFs show anti-correlated hard (16 - 30 keV) and soft (2 - 5 keV) X-ray delays of the order of a few tens to hundred seconds with a mean correlation coefficient of 0.42$\pm$0.11. Few observations shows correlated lags and on one occasion coincident with radio emission. We also report an anti-correlated hard X-ray delay of 113$\pm$51 s using the NuSTAR data of GX 17+2. Based on RXTE data, it was found that soft and hard X-ray fluxes are varying indicating the changes in the disk-corona structure during delays. We bridle the size of corona using relativistic precession, transition layer and boundary layer models. Assuming the delays to be readjustment time scale of disk-corona structure, height of the corona was estimated to be $\sim$ 17--100 km. Assuming that inner region of the truncated disk is occupied by the corona, we constrain the coronal readjustment velocities (v$_{corona}$=$\beta$ v$_{disk}$, where v$_{disk}$ is the radial velocity component of the disk) of the order of $\beta$=0.06-0.12. This study indicates that the observed delays are primarily dependent on the varying coronal readjustment velocities.

==> datafile_tex <==
OBSERVATION ID	&	START TIME	&	STOP TIME	&	EXPOSURE (s)	&	CC	&	CC ERROR	&	HR (position in HID)	&	LAG [ERROR in seconds]	\\
20056-02-01-00 	&	02/02/97 19:13	&	02/02/97 19:58	&	2452	&	0.857	&	0.059	&	 0.011-0.023	&	-                                                   	\\
20056-02-02-00       	&	06/02/97 22:46	&	07/02/97 00:01	&	2511	&	-0.376	&	0.126	&	 0.024-0.035 (II,III)   	&	 -468.007 [-547.3, -389.0]                              	\\
20053-03-02-00       	&	07/02/97 00:01	&	07/02/97 03:20	&	5940	&	 -                                                                   	&	-	&	 0.022-0.033    	&	 -                                                      	\\
20053-03-02-01       	&	08/02/97 03:35	&	08/02/97 05:52	&	32948	&	 -                                                                   	&	-	&	 0.022-0.033    	&	 -                                                      	\\
20053-03-02-02       	&	08/02/97 13:37	&	08/02/97 14:12	&	1082	&	 -                                                                   	&	-	&	 0.025-0.034    	&	 -                                                      	\\
20056-02-03-00       	&	10/02/97 00:08	&	10/02/97 00:58	&	2458	&	-0.431	&	0.124	&	 0.053-0.070    	&	 -                                                      	\\
20056-02-04-00       	&	13/02/97 03:39	&	13/02/97 05:14	&	2737	&	-0.385	&	0.128	&	 0.027-0.039    	&	 -                                                      	\\
20056-02-05-00       	&	15/02/97 06:56	&	15/02/97 07:36	&	2393	&	-0.299	&	0.095	&	 0.014-0.023    	&	 -                             	\\
20056-02-06-00       	&	18/02/97 00:20	&	18/02/97 01:00	&	2390	&	-0.402	&	0.113	&	 0.034-0.047 (II)   	&	 -300.969[-355.1,-248.4]                                                        	\\
20056-02-07-00       	&	23/02/97 23:09	&	24/02/97 00:12	&	2327	&	-0.309	&	0.08	&	 0.012-0.019    	&	 -                                                      	\\
20056-02-08-00       	&	27/02/97 02:19	&	27/02/97 03:34	&	2329	&	 -                                                                   	&	 -                                                     	&	 0.012-0.022    	&	 -                                                      	\\
20053-03-03-00 Sec A 	&	01/04/97 19:13	&	02/04/97 01:43	&	11471	&	0.525	&	0.091	&	 0.021-0.015    	&	 -                                                      	\\
“ Sec B              	&	“	&	"	&	"	&	0.935	&	0.028	&	 “              	&	 -                                                      	\\
“ Sec C              	&	“	&	"	&	"	&	0.827	&	0.068	&	 “              	&	 -                                                      	\\
“ Sec D              	&	“	&	"	&	"	&	0.561	&	0.012	&	 “              	&	 -                                                      	\\
20053-03-03-01 Sec A 	&	02/04/97 20:06	&	03/04/97 00:12	&	8920	&	-0.599	&	0.085	&	 0.060-0.037 (I,II)   	&	 -207.366 [-241.0,-174.9]                               	\\
“ Sec B              	&	“	&	"	&	"	&	-0.308	&	0.103	&	 “              	&	 -668.750[-739.7,-595.6]                                	\\
“ Sec C              	&	“	&	"	&	"	&	-0.478	&	0.111	&	 “              	&	 -100 [-75, 125]                                        	\\
20053-03-03-02 Sec A 	&	03/04/97 21:46	&	04/04/97 00:01	&	4967	&	-0.554	&	0.093	&	 0.036-0.057    	&	 -                                                      	\\
“ Sec B              	&	“	&	"	&	"	&	-0.575	&	0.136	&	 “              	&	 -                                                      	\\
20053-03-03-03 Sec A 	&	04/04/97 18:26	&	04/04/97 23:26	&	9862	&	 -                                                                   	&	 -                                                     	&	 0.024-0.040 (II,III)   	&	 ,-                                                     	\\
“ Sec B              	&	“	&	"	&	"	&	0.365	&	0.084	&	 “              	&	 1174.197 [1121.011,1226.001]                           	\\
“ Sec C              	&	“	&	"	&	"	&	 -                                                                   	&	 -                                                     	&	 “              	&	 -                                                      	\\
20053-03-01-00 Sec A 	&	27/07/97 02:13	&	27/07/97 08:02	&	11557	&	 -                                                                   	&	 -                                                     	&	 0.033-0.051    	&	 -                                                     	\\
“ Sec B              	&	“	&	"	&	"	&	-0.545	&	0.087	&	 “              	&	 -                                                     	\\
“ Sec C              	&	“	&	"	&	"	&	 -                                                                   	&	 -                                                     	&	 “              	&	 -                                                     	\\
“ Sec D              	&	“	&	"	&	"	&	-0.416	&	0.132	&	 “              	&	 -                                                     	\\
20053-03-01-01 Sec A 	&	27/07/97 16:41	&	27/07/97 19:09	&	21736	&	-0.48	&	0.101	&	 0.033-0.046 (II)    	&	 -228.646 [-269.9,-188.3]                               	\\
“ Sec B              	&	“	&	"	&	"	&	-0.341	&	-0.11	&	 “              	&	 -                                                      	\\
20053-03-01-02 Sec A 	&	27/07/97 20:01	&	28/07/97 00:33	&	9619	&	-0.757	&	0.067	&	 0.034-0.049    	&	 -                                                      	\\
“ Sec B              	&	“	&	"	&	"	&	-0.571	&	0.088	&	 “              	&	 -                                                      	\\
“ Sec C              	&	“	&	"	&	"	&	 -                                                                   	&	 -                                                     	&	 “              	&	 -                                                      	\\
30040-03-01-04       	&	07/08/98 06:40	&	07/08/98 08:10	&	2485	&	0.55	&	0.11	&	 0.014-0.022    	&	 -                                                      	\\
30040-03-01-00 Sec A 	&	07/08/98 11:28	&	07/08/98 19:09	&	17958	&	0.841	&	0.052	&	 0.013-0.026    	&	 -                                                      	\\
“ Sec B              	&	“	&	"	&	"	&	0.821	&	0.058	&	 “              	&	 -                                                      	\\
“ Sec C              	&	“	&	"	&	"	&	0.775	&	0.059	&	 “              	&	 -                                                      	\\
“ Sec D              	&	“	&	"	&	"	&	0.745	&	0.063	&	 “              	&	 -                                                      	\\
“ Sec E              	&	“	&	"	&	"	&	0.673	&	0.088	&	 “              	&	 -                                                      	\\
30040-03-01-02 Sec A 	&	07/08/98 19:33	&	08/08/98 01:16	&	12312	&	0.8	&	0.064	&	 0.012-0.024    	&	 -                                                      	\\
“ Sec B              	&	“	&	"	&	"	&	0.502	&	0.085	&	 “              	&	 -                                                      	\\
“ Sec C              	&	“	&	"	&	"	&	0.638	&	0.089	&	 “              	&	 -                                                      	\\
“ Sec D              	&	“	&	"	&	"	&	0.709	&	0.09	&	 “              	&	 -                                                      	\\
30040-03-01-01 Sec A 	&	08/08/98 12:55	&	08/08/98 19:09	&	28466	&	0.855	&	0.051	&	 0.013-0.049    	&	 -                                                      	\\
“ Sec B              	&	“	&	"	&	"	&	0.958	&	0.026	&	 “              	&	 -                                                      	\\
“ Sec C              	&	“	&	"	&	"	&	0.976	&	0.023	&	 “              	&	 -                                                      	\\
“ Sec D              	&	“	&	"	&	"	&	0.961	&	0.015	&	 “              	&	 -                                                      	\\
30040-03-01-03 Sec A 	&	08/08/98 19:33	&	08/08/98 23:40	&	9852	&	0.867	&	0.023	&	 0.023-0.066    	&	 -                                                      	\\
“ Sec B              	&	“	&	"	&	"	&	0.791	&	0.022	&	 “              	&	 -                                                      	\\
“ Sec C              	&	“	&	"	&	"	&	0.91	&	0.013	&	 “              	&	 -                                                      	\\
30040-03-02-00       	&	18/11/98 14:42	&	18/11/98 15:34	&	20707	&	0.633	&	0.084	&	 0.016-0.026    	&	 -                                                      	\\
30040-03-02-02       	&	18/11/98 20:57	&	18/11/98 21:54	&	2057	&	0.604	&	0.114	&	 0.014-0.027    	&	 -                                                      	\\
30040-03-02-01 Sec A 	&	19/11/98 14:28	&	19/11/98 18:25	&	42117	&	0.929	&	0.031	&	 0.013-0.042    	&	 -                                                      	\\
“ Sec B              	&	“	&	"	&	"	&	0.969	&	0.025	&	 “              	&	 -                                                      	\\
“ Sec C              	&	“	&	"	&	"	&	0.96	&	0.032	&	 “              	&	 -                                                      	\\
30040-03-02-03 Sec A 	&	20/11/98 00:17	&	20/11/98 06:55	&	13552	&	0.915	&	0.008	&	 0.012-0.064    	&	 -                                                      	\\
“ Sec B              	&	“	&	"	&	"	&	0.91	&	0.047	&	 “              	&	 -                                                      	\\
“ Sec C              	&	“	&	"	&	"	&	 -                                                                   	&	 -                                                     	&	 “              	&	 -                                                      	\\
“ Sec D              	&	“	&	"	&	"	&	0.594	&	0.088	&	 “              	&	 -                                                      	\\
30040-03-02-04 Sec A 	&	20/11/98 09:46	&	20/11/98 13:31	&	9134	&	0.897	&	0.015	&	 0.020-0.065    	&	 -                                                      	\\
“ Sec B              	&	“	&	"	&	"	&	0.891	&	0.017	&	 “              	&	 -                                                      	\\
“ Sec C              	&	“	&	"	&	"	&	0.909	&	0.028	&	 “              	&	 -                                                      	\\
40018-01-02-00 Sec A 	&	03/10/99 10:36	&	03/10/99 13:18	&	22780	&	 -                                                                   	&	 -                                                     	&	 0.039-0.060    	&	 -                                                      	\\
“ Sec B              	&	“	&	"	&	"	&	-0.628	&	0.091	&	 “              	&	 -                                                      	\\
40018-01-02-08 Sec A 	&	03/10/99 13:55	&	03/10/99 20:09	&	14156	&	-0.567	&	0.09	&	 0.032-0.064    	&	 -                                                      	\\
“ Sec B              	&	“	&	"	&	"	&	0.837	&	0.022	&	 “              	&	 -                                                      	\\
“ Sec C              	&	“	&	"	&	"	&	-0.308	&	0.11	&	 “              	&	 -                                                      	\\
“ Sec D              	&	“	&	"	&	"	&	-0.416	&	0.098	&	 “              	&	 -                                                      	\\
40018-01-02-20       	&	03/10/99 22:15	&	03/10/99 22:40	&	575	&	-0.417	&	0.264	&	 0.032-0.040    	&	 -                                                      	\\
40018-01-02-21       	&	03/10/99 23:30	&	04/10/99 00:09	&	1743	&	 -                                                                   	&	 -                                                     	&	 0.033-0.044    	&	 -                                                      	\\
40018-01-02-18       	&	04/10/99 02:54	&	04/10/99 03:42	&	1687	&	 -                                                                   	&	 -                                                     	&	 0.025-0.036    	&	 -                                                      	\\
40018-01-02-19 Sec A 	&	04/10/99 04:30	&	04/10/99 06:08	&	2944	&	 -                                                                   	&	 -                                                     	&	 0.024-0.036    	&	 -                                                      	\\
“ Sec B              	&	“	&	"	&	"	&	 -                                                                   	&	 -                                                     	&	 “              	&	 -                                                      	\\
40018-01-02-01 Sec A 	&	04/10/99 09:06	&	04/10/99 13:16	&	10661	&	0.486	&	0.104	&	 0.023-0.040    	&	 -                                                      	\\
“ Sec B              	&	“	&	"	&	"	&	 -                                                                   	&	 -                                                     	&	 “              	&	 -                                                      	\\
“ Sec C              	&	“	&	"	&	"	&	0.819	&	0.074	&	 “              	&	 -                                                      	\\
40018-01-02-11       	&	04/10/99 21:48	&	04/10/99 22:50	&	1680	&	 -                                                                   	&	 -                                                     	&	 0.038-0.049    	&	 -                                                      	\\
40018-01-02-23       	&	04/10/99 23:30	&	05/10/99 00:21	&	1575	&	 -                                                                   	&	 -                                                     	&	 0.045-0.057    	&	 -                                                      	\\
40018-01-02-10       	&	05/10/99 02:51	&	05/10/99 03:40	&	1750	&	-0.414	&	0.183	&	 0.055-0.070    	&	 -                                                      	\\
40018-01-02-17       	&	05/10/99 04:27	&	05/10/99 05:20	&	2170	&	-0.368	&	0.148	&	 0.056-0.074    	&	 -                                                      	\\
40018-01-02-22       	&	05/10/99 05:56	&	05/10/99 06:05	&	533	&	 -                                                                   	&	 -                                                     	&	 0.060-0.072    	&	 -                                                      	\\
40018-01-02-03 Sec A 	&	05/10/99 09:04	&	05/10/99 12:07	&	7065	&	-0.597	&	0.086	&	 0.054-0.087    	&	 -                                                      	\\
“ Sec B              	&	“	&	"	&	"	&	-0.403	&	0.102	&	 “              	&	 -                                                      	\\
40018-01-02-02 Sec A 	&	05/10/99 13:52	&	05/10/99 18:29	&	10557	&	-0.633	&	0.095	&	 0.052-0.079    	&	 -                                                      	\\
“ Sec B              	&	“	&	"	&	"	&	 -                                                                   	&	 -                                                     	&	 “              	&	 -                                                      	\\
“ Sec C              	&	“	&	"	&	"	&	 -                                                                   	&	 -                                                     	&	 “              	&	 -                                                      	\\
40018-01-02-15       	&	05/10/99 20:26	&	05/10/99 20:56	&	909	&	 -                                                                   	&	 -                                                     	&	 0.036-0.048    	&	 -                                                      	\\
40018-01-02-12       	&	05/10/99 23:37	&	06/10/99 00:11	&	926	&	0.917	&	0.042	&	 0.033-0.076    	&	 -                                                      	\\
40018-01-02-16       	&	06/10/99 01:21	&	06/10/99 01:56	&	849	&	 -                                                                   	&	 -                                                     	&	 0.033-0.041    	&	 -                                                      	\\
40018-01-02-05 Sec A 	&	“	&	06/10/99 13:12	&	12522	&	-0.394	&	0.154	&	 0.033-0.062  (I,II)  	&	- 	\\
“ Sec B              	&	“	&	"	&	"	&	-0.557	&	0.091	&	 “              	&	 -293.754242 [-340.5,250.7]                             	\\
“ Sec C              	&	“	&	"	&	"	&	-0.557	&	0.091	&	 “              	&	-	\\
“ Sec D              	&	“	&	"	&	"	&	-0.427	&	0.137	&	 “              	&	 -98.125061 [-160.1,-39.09]                              	\\
“ Sec E              	&	“	&	"	&	"	&	-0.427	&	0.137	&	 “              	&	 279.260895 [235.0, 323.7]                              	\\
40018-01-02-28       	&	06/10/99 20:13	&	06/10/99 20:53	&	1485	&	 -                                                                   	&	 -                                                     	&	 0.025-0.033    	&	-	\\
40018-01-02-26       	&	06/10/99 21:49	&	06/10/99 22:32	&	1461	&	 -                                                                   	&	 -                                                     	&	 0.021-0.031    	&	-	\\
40018-01-02-27       	&	06/10/99 23:25	&	07/10/99 00:01	&	1602	&	0.74	&	0.123	&	 0.022-0.032    	&	-	\\
40018-01-02-09 Sec A 	&	07/10/99 02:38	&	07/10/99 07:00	&	8475	&	0.767	&	0.101	&	 0.018-0.034    	&	-	\\
“ Sec B              	&	“	&	"	&	"	&	0.747	&	0.089	&	 “              	&	-	\\
“ Sec C              	&	“	&	"	&	"	&	 -                                                                   	&	 -                                                     	&	 “              	&	-	\\
40018-01-02-24       	&	07/10/99 07:50	&	07/10/99 08:35	&	1966	&	0.679	&	0.145	&	 0.020-0.030    	&	-	\\
40018-01-02-06 Sec A 	&	07/10/99 09:12	&	07/10/99 13:10	&	9725	&	0.72	&	0.07	&	 0.017-0.036    	&	-	\\
“ Sec B              	&	“	&	"	&	"	&	0.401	&	0.105	&	 “              	&	-	\\
“ Sec C              	&	“	&	"	&	"	&	 -                                                                   	&	 -                                                     	&	 “              	&	-	\\
40018-01-02-29 Sec A 	&	07/10/99 21:48	&	08/10/99 00:01	&	2939	&	 -                                                                   	&	 -                                                     	&	 0.031-0.043    	&	-	\\
“ Sec B              	&	“	&	"	&	"	&	 -                                                                   	&	 -                                                     	&	 “              	&	-	\\
40018-01-01-00       	&	08/10/99 01:11	&	08/10/99 01:54	&	1285	&	 -                                                                   	&	 -                                                     	&	 0.048-0.038    	&	-	\\
40018-01-01-01       	&	08/10/99 02:51	&	08/10/99 04:08	&	1455	&	 -                                                                   	&	 -                                                     	&	 0.035-0.046    	&	-	\\
40018-01-01-02 Sec A 	&	08/10/99 04:31	&	08/10/99 07:57	&	6819	&	-0.3	&	0.196	&	 0.032-0.049    	&	-	\\
“ Sec B              	&	“	&	"	&	"	&	-0.413	&	0.128	&	 “              	&	-	\\
“ Sec C              	&	“	&	"	&	"	&	 -                                                                   	&	 -                                                     	&	 “              	&	-	\\
40018-01-01-03 Sec A 	&	08/10/99 08:58	&	08/10/99 12:05	&	7007	&	-0.439	&	0.099	&	 0.036-0.054    	&	-	\\
“ Sec B              	&	“	&	"	&	"	&	 -                                                                   	&	 -                                                     	&	 “              	&	-	\\
40018-01-01-04 Sec A 	&	08/10/99 13:47	&	08/10/99 19:12	&	11159	&	-0.344	&	0.159	&	 0.060-0.037    	&	-	\\
“ Sec B              	&	“	&	"	&	"	&	-0.222	&	0.137	&	 “              	&	-	\\
“ Sec C              	&	“	&	"	&	"	&	-0.668	&	0.114	&	 “              	&	-	\\
“ Sec D              	&	“	&	"	&	"	&	-0.335	&	0.192	&	 “              	&	-	\\
40018-01-03-09       	&	08/10/99 20:09	&	08/10/99 20:50	&	1301	&	 -                                                                   	&	 -                                                     	&	 0.041-0.052    	&	-	\\
40018-01-03-17       	&	08/10/99 21:46	&	08/10/99 22:33	&	1190	&	                                                                     	&	                                                       	&	 0.042-0.055    	&	-	\\
40018-01-01-05       	&	08/10/99 23:21	&	09/10/99 00:04	&	1661	&	                                                                     	&	                                                       	&	 0.043-0.053    	&	-	\\
40018-01-01-06       	&	09/10/99 00:57	&	09/10/99 01:54	&	2080	&	                                                                     	&	                                                       	&	 0.039-0.050    	&	-	\\
40018-01-01-07       	&	09/10/99 02:33	&	09/10/99 03:34	&	2440	&	-0.334	&	0.131	&	 0.037-0.053    	&	-	\\
40018-01-01-08 Sec A 	&	09/10/99 04:10	&	09/10/99 09:31	&	11756	&	-0.391	&	0.119	&	 0.029-0.046 (II)    	&	 -233.187622 [-282.5,-180.1]                            	\\
“ Sec B              	&	“	&	"	&	"	&	 -                                                                   	&	 -                                                     	&	 “              	&	-	\\
“ Sec C              	&	“	&	"	&	"	&	 -                                                                   	&	 -                                                     	&	 “              	&	-	\\
“ Sec D              	&	“	&	"	&	"	&	 -                                                                   	&	 -                                                     	&	 “              	&	-	\\
40018-01-01-09       	&	09/10/99 10:32	&	09/10/99 11:30	&	3464	&	 -                                                                   	&	 -                                                     	&	 0.026-0.038    	&	-	\\
40018-01-01-10 Sec A 	&	09/10/99 12:09	&	09/10/99 16:18	&	10377	&	0.911	&	0.03	&	 0.016-0.068    	&	-	\\
“ Sec B              	&	“	&	"	&	"	&	0.459	&	0.1	&	 “              	&	-	\\
“ Sec C              	&	“	&	"	&	"	&	0.552	&	0.093	&	 “              	&	-	\\
40018-01-01-11       	&	09/10/99 17:34	&	09/10/99 18:04	&	1152	&	0.759	&	0.155	&	 0.019-0.028    	&	-	\\
40018-01-01-12       	&	09/10/99 20:07	&	09/10/99 20:50	&	1188	&	0.477	&	0.204	&	 0.023-0.045    	&	-	\\
40018-01-01-13       	&	09/10/99 21:44	&	09/10/99 22:27	&	1200	&	0.508	&	0.183	&	 0.020-0.029    	&	-	\\
40018-01-03-01       	&	10/10/99 02:41	&	10/10/99 03:26	&	1817	&	0.496	&	0.136	&	 0.016-0.027    	&	-	\\
40018-01-01-14       	&	10/10/99 04:29	&	10/10/99 05:10	&	1521	&	0.446	&	0.141	&	 0.016-0.027    	&	-	\\
40018-01-03-02 Sec A 	&	10/10/99 05:55	&	10/10/99 11:28	&	12932	&	0.921	&	0.045	&	 0.017-0.047    	&	-	\\
“ Sec B              	&	“	&	"	&	"	&	0.971	&	0.02	&	 “              	&	-	\\
“ Sec C              	&	“	&	"	&	"	&	0.904	&	0.036	&	 “              	&	-	\\
“ Sec D              	&	“	&	"	&	"	&	0.906	&	0.043	&	 “              	&	-	\\
40018-01-03-03       	&	10/10/99 12:07	&	10/10/99 12:57	&	3016	&	0.966	&	0.023	&	 0.022-0.049    	&	-	\\
40018-01-03-04 Sec A 	&	10/10/99 15:18	&	10/10/99 19:09	&	6828	&	0.764	&	0.094	&	 0.015-0.028    	&	-	\\
“ Sec B              	&	“	&	"	&	"	&	0.607	&	0.177	&	 “              	&	-	\\
“ Sec C              	&	“	&	"	&	"	&	0.928	&	0.106	&	 “              	&	-	\\
“ Sec D              	&	“	&	"	&	"	&	0.684	&	0.131	&	 “              	&	-	\\
40018-01-01-16       	&	10/10/99 20:05	&	10/10/99 20:49	&	1068	&	0.723	&	0.059	&	 0.040-0.068    	&	-	\\
40018-01-03-05       	&	10/10/99 21:41	&	10/10/99 22:27	&	1235	&	0.88	&	0.089	&	 0.030-0.040    	&	-	\\
40018-01-03-06       	&	10/10/99 23:18	&	11/10/99 00:06	&	1620	&	0.925	&	0.065	&	 0.019-0.031    	&	-	\\
40018-01-01-15       	&	11/10/99 01:03	&	11/10/99 01:30	&	1453	&	0.953	&	0.051	&	 0.020-0.036    	&	-	\\
40018-01-03-07       	&	11/10/99 02:32	&	11/10/99 03:19	&	2306	&	0.921	&	0.054	&	 0.014-0.029    	&	-	\\
40018-01-03-08 Sec A 	&	11/10/99 04:18	&	11/10/99 09:13	&	10080	&	0.895	&	0.055	&	 0.019-0.074    	&	-	\\
“ Sec B              	&	“	&	"	&	"	&	0.887	&	0.021	&	 “              	&	-	\\
“ Sec C              	&	“	&	"	&	"	&	0.961	&	0.011	&	 “              	&	-	\\
“ Sec D              	&	“	&	"	&	"	&	0.957	&	0.055	&	 “              	&	-	\\
40018-01-03-10 Sec A 	&	11/10/99 10:46	&	11/10/99 13:02	&	5841	&	-	&	-	&	 “              	&	-	\\
“ Sec B              	&	“	&	"	&	"	&	0.504	&	0.093	&	 0.014-0.027    	&	-	\\
40018-01-03-11 Sec A 	&	11/10/99 13:41	&	11/10/99 16:16	&	6660	&	0.91	&	0.046	&	 0.015-0.029    	&	-	\\
“ Sec B              	&	“	&	"	&	"	&	0.814	&	0.065	&	 “              	&	-	\\
40018-01-03-12       	&	11/10/99 17:30	&	11/10/99 18:18	&	1144	&	0.889	&	0.091	&	 0.020-0.031    	&	-	\\
40018-01-03-13       	&	11/10/99 20:03	&	11/10/99 20:42	&	941	&	0.829	&	0.129	&	 0.018-0.028    	&	-	\\
40018-01-03-14       	&	11/10/99 21:39	&	11/10/99 22:20	&	1301	&	0.95	&	0.062	&	 0.020-0.035    	&	-	\\
40018-01-03-15       	&	11/10/99 23:15	&	12/10/99 00:03	&	1721	&	0.953	&	0.045	&	 0.025-0.040    	&	-	\\
40018-01-03-16       	&	12/10/99 00:51	&	12/10/99 01:46	&	2081	&	0.789	&	0.082	&	 0.016-0.027    	&	-	\\
40018-01-01-17       	&	12/10/99 02:27	&	12/10/99 03:43	&	2461	&	0.971	&	0.022	&	 0.019-0.052    	&	-	\\
40018-01-01-18 Sec A 	&	12/10/99 04:14	&	12/10/99 07:06	&	5464	&	0.767	&	0.085	&	 0.018-0.041    	&	-	\\
“ Sec B              	&	“	&	"	&	"	&	0.952	&	0.029	&	 “              	&	-	\\
40018-01-03-00       	&	31/03/00 12:16	&	31/03/00 12:48	&	1746	&	0.833	&	0.065	&	 0.018-0.031    	&	-	\\
40018-01-03-18       	&	31/03/00 13:51	&	31/03/00 14:29	&	2229	&	 -                                                                   	&	 -                                                     	&	 0.014-0.028    	&	-	\\
40018-01-03-19 Sec A 	&	31/03/00 15:27	&	31/03/00 16:32	&	2978	&	0.755	&	0.101	&	 0.014-0.026    	&	-	\\
“ Sec B              	&	“	&	"	&	"	&	0.655	&	0.192	&	 “              	&	-	\\
70023-01-01-01 Sec A 	&	04/11/02 18:18	&	04/11/02 22:00	&	8937	&	0.621	&	0.109	&	 0.046-0.064 (I)   	&	 113.878502 [88.84,139]                                 	\\
“ Sec B              	&	“	&	"	&	"	&	-0.3	&	0.113	&	 “              	&	-	\\
“ Sec C              	&	“	&	"	&	"	&	-0.452	&	0.117	&	 “              	&	 -168.6763153 [-200.4, -50.795]                          	\\
70023-01-01-03       	&	04/11/02 22:36	&	04/11/02 23:34	&	3450	&	 -                                                                   	&	 -                                                     	&	 0.048-0.059    	&	-                                             	\\
70023-01-01-00 Sec A 	&	05/11/02 00:27	&	05/11/02 06:34	&	12715	&	-0.259	&	0.089	&	 0.046-0.064 (I)   	&	 -265.393066[-342.1,-191.0]                             	\\
“ Sec B              	&	“	&	"	&	"	&	 -                                                                   	&	 -                                                     	&	 “              	&	-	\\
“ Sec C              	&	“	&	"	&	"	&	-0.268	&	0.11	&	 “              	&	 -451.493591[-529.5,373.5]                              	\\
“ Sec D              	&	“	&	"	&	"	&	-0.367	&	0.103	&	 “              	&	 -175.953293 [-240.8, -111.3]                           	\\
70023-01-02-00 Sec A 	&	09/11/02 18:10	&	09/11/02 23:44	&	13615	&	0.878	&	0.018	&	 0.012-0.054    	&	-	\\
“ Sec B              	&	“	&	"	&	"	&	0.965	&	0.026	&	 “              	&	-	\\
“ Sec C              	&	“	&	"	&	"	&	0.686	&	0.071	&	 “              	&	-	\\
“ Sec D              	&	“	&	"	&	"	&	0.468	&	0.099	&	 “              	&	-	\\
70023-01-02-01 Sec A 	&	10/11/02 00:39	&	10/11/02 06:26	&	12714	&	0.499	&	0.118	&	 0.013-0.023    	&	-	\\
“ Sec B              	&	“	&	"	&	"	&	0.887	&	0.05	&	 “              	&	-	\\
“ Sec C              	&	“	&	"	&	"	&	 -                                                                   	&	 -                                                     	&	 “              	&	-	\\
“ Sec D              	&	“	&	"	&	"	&	0.619	&	0.083	&	 “              	&	-	\\
70023-01-03-01 Sec A 	&	15/11/02 22:39	&	16/11/02 06:11	&	15374	&	0.378	&	0.133	&	 0.024-0.035    	&	-	\\
“ Sec B              	&	“	&	"	&	"	&	-0.425	&	0.133	&	 “              	&	-	\\
“ Sec C              	&	“	&	"	&	"	&	-0.282	&	0.13	&	 “              	&	-	\\
“ Sec D              	&	“	&	"	&	"	&	 -                                                                   	&	 -                                                     	&	 “              	&	-	\\
“ Sec E              	&	“	&	"	&	"	&	-0.433	&	0.087	&	 “              	&	-	\\
80022-01-01-07       	&	26/03/04 03:06	&	26/03/04 03:35	&	1683	&	 -                                                                   	&	 -                                                     	&	 0.018-0.023    	&	-	\\
80022-01-01-09       	&	26/03/04 08:00	&	26/03/04 08:22	&	1284	&	0.505	&	0.187	&	 0.020-0.026    	&	-	\\
80022-01-01-10       	&	23/03/04 09:36	&	26/03/04 10:00	&	1166	&	 -                                                                   	&	 -                                                     	&	 0.021-0.027    	&	-	\\
80022-01-01-11       	&	26/03/04 11:04	&	26/03/04 11:51	&	1560	&	0.461	&	0.182	&	 0.019-0.025    	&	-	\\
80022-01-01-00       	&	27/03/04 21:24	&	27/03/04 21:58	&	2037	&	 -                                                                   	&	 -                                                     	&	 0.031-0.037    	&	-	\\
80022-01-01-12       	&	28/03/04 03:57	&	28/03/04 04:15	&	1027	&	 -                                                                   	&	 -                                                     	&	 0.025-0.033    	&	-	\\
80022-01-01-13       	&	28/03/04 05:36	&	28/03/04 05:52	&	945	&	 -                                                                   	&	 -                                                     	&	 0.026-0.031    	&	-	\\
80022-01-01-14       	&	28/03/04 08:48	&	28/03/04 09:16	&	1391	&	 -                                                                   	&	 -                                                     	&	 0.022-0.028    	&	-	\\
80022-01-01-15       	&	28/03/04 10:16	&	28/03/04 11:06	&	1801	&	0.476	&	0.131	&	 0.020-0.026    	&	-	\\
80022-01-01-05 Sec A 	&	28/03/04 17:43	&	28/03/04 22:26	&	9652	&	0.915	&	0.042	&	 0.014-0.056    	&	-	\\
“ Sec B              	&	“	&	"	&	"	&	0.868	&	0.015	&	 “              	&	-	\\
“ Sec C              	&	“	&	"	&	"	&	0.924	&	0.024	&	 “              	&	-	\\
80022-01-01-16       	&	29/03/04 06:50	&	29/03/04 07:30	&	1554	&	0.878	&	0.091	&	 0.015-0.021    	&	-	\\
80022-01-01-03 Sec A 	&	29/03/04 20:35	&	29/03/04 22:43	&	4553	&	0.925	&	0.009	&	 0.014-0.056    	&	-	\\
“ Sec B              	&	“	&	"	&	"	&	0.93	&	0.058	&	 “              	&	-	\\
80022-01-01-04 Sec A 	&	30/03/04 23:32	&	31/03/04 01:42	&	4492	&	0.637	&	0.105	&	 0.015-0.023    	&	-	\\
“ Sec B              	&	“	&	"	&	"	&	 -                                                                   	&	 -                                                     	&	 “              	&	-	\\
80022-01-01-02 Sec A 	&	31/03/04 17:03	&	31/03/04 22:40	&	11149	&	 -                                                                   	&	 -                                                     	&	 0.028-0.063    	&	-	\\
“ Sec B              	&	“	&	"	&	"	&	0.917	&	0.025	&	 “              	&	-	\\
“ Sec C              	&	“	&	"	&	"	&	 -                                                                   	&	 -                                                     	&	 “              	&	-	\\
“ Sec D              	&	“	&	"	&	"	&	-0.247	&	0.15	&	 “              	&	-	\\
80022-01-01-06       	&	01/04/04 13:07	&	01/04/04 14:31	&	-	&	                                                                     	&	                                                       	&	 “              	&	-	\\
80022-01-01-01 Sec A 	&	01/04/04 16:10	&	01/04/04 20:52	&	10329	&	-	&	-	&	 0.026-0.040 (II,III)   	&	-	\\
“ Sec B              	&	“	&	"	&	"	&	-0.418	&	0.095	&	 “              	&	 -497.211609 [-549.8, -444.6]                           	\\
“ Sec C              	&	“	&	"	&	"	&	-0.488	&	0.106	&	 “              	&	-	\\
90022-07-01-01       	&	07/04/04 22:00	&	07/04/04 22:15	&	849	&	0.952	&	0.021	&	 0.023-0.047    	&	-	\\
80022-01-02-00 Sec A 	&	11/05/04 10:58	&	11/05/04 18:58	&	17086	&	-0.461	&	0.126	&	 0.026-0.038 (II,III)   	&	-	\\
“ Sec B              	&	“	&	"	&	"	&	-0.474	&	0.092	&	 “              	&	 -365.052185[-419.4, -315.0]                            	\\
“ Sec C              	&	“	&	"	&	"	&	-0.421	&	0.106	&	 “              	&	 1072.51172[1009.0, 1134.0]                             	\\
“ Sec D              	&	“	&	"	&	"	&	0.532	&	0.099	&	 “              	&	 549.988464 [501.3, 598.6]                              	\\
“ Sec E              	&	“	&	"	&	"	&	0.384	&	0.117	&	 “              	&	 -680.401733 [-765.6, -605.6]                           	\\
80022-01-02-01 Sec A 	&	12/05/04 10:35	&	12/05/04 15:02	&	10247	&	 -                                                                   	&	 -                                                     	&	 0.022-0.033 (II,III,IV)   	&	-	\\
“ Sec B              	&	“	&	"	&	"	&	-0.25	&	0.092	&	 “              	&	 1506.20361 [1364.0, 1638.0]                            	\\
“ Sec C              	&	“	&	"	&	"	&	-0.275	&	0.092	&	 “              	&	 1166.8501[1082.0, 1252.0]                              	\\
80022-01-02-02       	&	12/05/04 18:28	&	12/05/04 19:15	&	2216	&	 -                                                                   	&	 -                                                     	&	 0.019-0.024    	&	-	\\
80022-01-03-00       	&	22/05/04 04:09	&	22/05/04 04:25	&	903	&	0.73	&	0.21	&	 0.022-0.026    	&	-	\\
80022-01-03-03       	&	22/05/04 22:56	&	22/05/04 23:22	&	1509	&	 -                                                                   	&	 -                                                     	&	 0.024-0.029    	&	-	\\
80022-01-03-05       	&	24/05/04 00:10	&	24/05/04 00:43	&	1939	&	0.447	&	0.144	&	 0.022-0.029    	&	-	\\
80022-01-03-08 Sec A 	&	24/05/04 15:52	&	24/05/04 18:42	&	5436	&	-0.385	&	0.121	&	 0.026-0.038 (II,III)   	&	 -454.601715 [-506.0,-396.8]                            	\\
“ Sec B              	&	“	&	"	&	"	&	-0.303	&	0.117	&	 “              	&	-	\\
80022-01-03-06       	&	24/05/04 19:15	&	24/05/04 20:07	&	1584	&		&	-	&	 0.023-0.031    	&	-	\\
80022-01-03-10       	&	25/05/04 20:07	&	25/05/04 21:40	&	2790	&	 -                                                                   	&	 -                                                     	&	 0.027-0.034    	&	-	\\
80022-01-04-00 Sec A 	&	21/06/04 14:41	&	21/06/04 20:31	&	13556	&	0.858	&	0.059	&	 0.013-0.028    	&	-	\\
“ Sec B              	&	“	&	"	&	"	&	0.893	&	0.045	&	 “              	&	-	\\
“ Sec C              	&	“	&	"	&	"	&	0.786	&	0.071	&	 “              	&	-	\\
“ Sec D              	&	“	&	"	&	"	&	0.688	&	0.075	&	 “              	&	-	\\
80022-01-05-00 Sec A 	&	26/06/04 09:36	&	26/06/04 16:27	&	15654	&	-0.301	&	0.1	&	 0.031-0.047 (II)   	&	-	\\
“ Sec B              	&	“	&	"	&	"	&	-0.287	&	0.127	&	 “              	&	 261.267853 [141.9, 381.9]                              	\\
“ Sec C              	&	“	&	"	&	"	&	-0.259	&	-0.095	&	 “              	&	    1018.25555 [926.4,  1096]                                                    	\\
“ Sec D              	&	“	&	"	&	"	&	-0.359	&	0.111	&	 “              	&	 -103.23452 [-150.9, -56.08]                            	\\
“ Sec E              	&	“	&	"	&	"	&	0.453	&	-0.121	&	 “              	&	  523.190674 [480.8, 566.3]                                                      	\\
90022-07-02-00       	&	21/08/04 02:44	&	21/08/04 03:12	&	1645	&	0.974	&	0.032	&	 0.016-0.029    	&	-	\\
90022-07-03-00       	&	29/08/04 01:44	&	29/08/04 02:15	&	1710	&	0.928	&	0.02	&	 0.024-0.057    	&	-	\\
90022-07-04-01       	&	08/10/04 13:22	&	08/10/04 13:52	&	1739	&	-0.409	&	-0.164	&	 0.036-0.044  (II)  	&	 -251.259857 [-347.9, -157.5]                           	\\
90022-07-04-02       	&	08/10/04 15:01	&	08/10/04 15:26	&	1440	&	-0.477	&	0.181	&	 0.042-0.050    	&	-	\\
90022-07-04-00 Sec A 	&	10/10/04 01:08	&	10/10/04 04:14	&	6781	&	-0.551	&	0.104	&	 0.050-0.061    	&	-	\\
“ Sec B              	&	“	&	"	&	"	&	-0.424	&	0.096	&	 “              	&	-	\\
90022-07-05-01       	&	08/10/05 11:19	&	08/10/05 11:59	&	2372	&	 -                                                                   	&	 -                                                     	&	 0.027-0.034    	&	-	\\
90022-07-05-03       	&	08/10/05 16:13	&	08/10/05 16:42	&	1718	&	 -                                                                   	&	 -                                                     	&	 0.032-0.046    	&	-	\\
90022-07-05-02       	&	08/10/05 17:50	&	08/10/05 18:16	&	1539	&	-0.407	&	0.147	&	 0.032-0.047 (II)   	&	 -132.433868 [-196.2, -71.02]                           	\\
91152-02-01-00 Sec A 	&	10/05/06 05:25	&	10/05/06 08:06	&	14111	&	 -                                                                   	&	 -                                                     	&	 0.026-0.042 (II,III)   	&	-	\\
“ Sec B              	&	“	&	"	&	"	&	-0.552	&	0.076	&	 “              	&	 187.787186[152.5, 225.3]                               	\\
“ Sec C              	&	“	&	"	&	"	&	0.322	&	0.112	&	 “              	&	 391.58963 [320.4, 488.4]                               	\\
“ Sec D              	&	“	&	"	&	"	&	-0.263	&	0.104	&	 “              	&	 -125.240318 [-222.8, 24.42]                            	\\
91152-02-01-01       	&	10/05/06 08:42	&	10/05/06 08:57	&	850	&	 -                                                                   	&	 -                                                     	&	 0.024-0.034    	&	-	\\
92042-01-03-00       	&	07/07/06 03:13	&	07/07/06 03:46	&	1595	&	0.791	&	0.096	&	 0.012-0.024    	&	-	\\
92042-01-03-01       	&	07/07/06 04:42	&	07/07/06 05:31	&	2027	&	 -                                                                   	&	 -                                                     	&	 0.017-0.026    	&	-	\\
92042-01-03-02       	&	07/07/06 06:21	&	07/07/06 06:59	&	1834	&	0.399	&	0.168	&	 0.017-0.025  (IV)  	&	 -134.524612 [-212.7, -56.05]                           	\\
92042-01-04-00       	&	12/07/06 08:59	&	12/07/06 09:43	&	2092	&	0.792	&	0.083	&	 0.019-0.029    	&	-	\\
92042-01-05-00       	&	14/07/06 03:22	&	14/07/06 03:56	&	1247	&	 -                                                                   	&	 -                                                     	&	 0.018-0.026    	&	-	\\
92042-01-05-01       	&	14/07/06 04:55	&	14/07/06 05:42	&	1453	&	0.583	&	0.137	&	 0.016-0.026    	&	-	\\
92042-01-05-02       	&	14/07/06 06:30	&	14/07/06 07:16	&	1781	&	0.696	&	0.104	&	 0.014-0.023    	&	-	\\
92042-01-05-03       	&	14/07/06 08:03	&	14/07/06 08:50	&	2233	&	0.434	&	0.132	&	 0.015-0.023    	&	-	\\
91152-02-02-00       	&	19/08/06 22:37	&	20/08/06 04:20	&	13352	&	0.806	&	0.03	&	 0.012-0.024    	&	-	\\
93406-11-01-00       	&	04/07/07 16:01	&	04/07/07 17:25	&	3255	&	0.911	&	0.043	&	 0.015-0.028    	&	-	\\
90022-07-06-01       	&	19/09/07 09:11	&	19/09/07 10:45	&	2944	&	0.431	&	0.111	&	 0.016-0.025    	&	-	\\
93071-03-01-00 Sec A 	&	10/05/08 05:04	&	10/05/08 06:21	&	1154	&	0.628	&	0.277	&	 0.015-0.024    	&	-	\\
“ Sec B              	&	“	&	"	&	"	&	 -                                                                   	&	 -                                                     	&	 “              	&	-	\\
93439-01-01-00 Sec A 	&	23/05/08 07:08	&	23/05/08 09:01	&	3503	&	 -                                                                   	&	 -                                                     	&	 0.020-0.034    	&	-	\\
“ Sec B              	&	“	&	"	&	"	&	 -                                                                   	&	 -                                                     	&	 “              	&	-	\\
“ Sec C              	&	“	&	"	&	"	&	 -                                                                   	&	 -                                                     	&	 “              	&	-	\\
93439-01-02-00 Sec A 	&	27/05/08 05:52	&	27/05/08 07:52	&	4941	&	-0.48	&	0.167	&	 0.041-0.061 (I,II)   	&	 -192.779831 [-243.4, -144.0]                           	\\
“ Sec B              	&	“	&	"	&	"	&	-0.376	&	0.149	&	 “              	&	 -186.520447 [-250.7, -122.3]                           	\\
“ Sec C              	&	“	&	"	&	"	&	 -                                                                   	&	 -                                                     	&	 “              	&	-	\\
93439-01-04-00 Sec A 	&	02/06/08 04:14	&	02/06/08 08:11	&	9913	&	 -                                                                   	&	 -                                                     	&	 0.017-0.036    	&	-	\\
“ Sec B              	&	“	&	"	&	"	&	 -                                                                   	&	 -                                                     	&	 “              	&	-	\\
“ Sec C              	&	“	&	"	&	"	&	0.716	&	0.093	&	 “              	&	-	\\
93439-01-05-00       	&	18/07/08 04:13	&	18/07/08 05:27	&	3374	&	-0.454	&	0.117	&	 0.033-0.046    	&	-	\\
93439-01-05-01       	&	19/07/08 03:45	&	19/07/08 04:51	&	3486	&	-0.609	&	0.088	&	 0.030-0.044 (II,III)   	&	 -267.974731[-295.0, -241.0]                            	\\
93439-01-05-02       	&	23/07/08 02:00	&	23/07/08 03:04	&	3445	&	-0.388	&	0.101	&	 0.035-0.049    	&	-	\\
93439-01-06-00 Sec A 	&	27/07/08 01:48	&	27/07/08 04:43	&	7065	&	0.963	&	0.025	&	 0.018-0.058    	&	-	\\
“ Sec B              	&	“	&	"	&	"	&	0.888	&	0.013	&	 “              	&	-	\\
93071-03-02-00       	&	21/10/08 06:02	&	21/10/08 06:50	&	2848	&	-0.385	&	0.11	&	 0.040-0.054 (I,II)   	&	 -691.908142[-749.1, -635.8 ]                          	\\


